Going Beyond RF: How AI-enabled Multimodal Beamforming will Shape the NextG Standard

Incorporating artificial intelligence and machine learning (AI/ML) methods within the 5G wireless standard promises autonomous network behavior and ultra-low-latency reconfiguration. However, the effort so far has purely focused on learning from radio frequency (RF) signals. Future standards and next-generation (nextG) networks beyond 5G will have two significant evolutions over the state-of-the-art 5G implementations: (i) massive number of antenna elements, scaling up to hundreds-to-thousands in number, and (ii) inclusion of AI/ML in the critical path of the network reconfiguration process that can access sensor feeds from a variety of RF and non-RF sources. While the former allows unprecedented flexibility in 'beamforming', where signals combine constructively at a target receiver, the latter enables the network with enhanced situation awareness not captured by a single and isolated data modality. This survey presents a thorough analysis of the different approaches used for beamforming today, focusing on mmWave bands, and then proceeds to make a compelling case for considering non-RF sensor data from multiple modalities, such as LiDAR, Radar, GPS for increasing beamforming directional accuracy and reducing processing time. This so called idea of multimodal beamforming will require deep learning based fusion techniques, which will serve to augment the current RF-only and classical signal processing methods that do not scale well for massive antenna arrays. The survey describes relevant deep learning architectures for multimodal beamforming, identifies computational challenges and the role of edge computing in this process, dataset generation tools, and finally, lists open challenges that the community should tackle to realize this transformative vision of the future of beamforming.

==> Sections/Beamforming_5G.tex <==
\section{Beamforming in 5G NR }
% \add{Debashri}
\label{sec:beamforming_5g_nr}
The new air interface 5G NR for 5G network is already supporting different 5G frequency bands depending on locations~\cite{3gpp_5gnr}. 5G NR is aimed to be global standard for the wireless communication of 3GPP 5G networks~\cite{atis_2020}. 5G NR supports the frequency bands from different ranges: sub-1 GHz, sub-6 GHz, sub-30 GHz, as well as above-30 GHz~\cite{Rumyancev_2019}. We call the first three as sub-mmWave and the above-30 GHz as mmWave band. In that regard, first we give a fleeting glance on beamforming techniques in sub-mmWave and then we dive in mmWave band.

% While beamforming can be used in sub-6 GHz band mMIMO it is become a necessity in above 6 GHz band due to different propagation characteristics, such as high free space path loss, absorption by atmospheric gases and rain and non-line of sight propagation. Some comparison of physical, practical and use-case differences between mMIMO systems in sub- and above 6 GHz is presented in~\cite{Bjornson_2019}.

\subsection{Using the Sub-mmWave Band} 
Exploiting the low propagation loss characteristics the sub-1 GHz band is used for better area coverage in urban and rural areas, as well as for indoor penetration. In the sub-1 GHz frequency coexists with the LTE framework. In United States, Verizon, AT\&T, T-Mobile got assigned to either of 600MHz or 850 MHz band. Next for Sub-6 GHz band offers a good tradeoff between equipment size, range and capacity. Sub-6 GHz is by far the most common widely used band with data rate of 100-400 Mbit/s, but has better range than mmWave, especially outdoors~\cite{cnet_2019}. For the additional capacity and higher data rate, the n257 (26.5-29.5 GHz), n258 (24.25-27.5 GHz), and n261 (27.5-28.35 GHz) bands are also supported in 5G NR standard~\cite{3gpp_5gnr}.  However, the requirement of supporting multiGbps communication in 5G can not be achieved by sub-mmWave bands. 

% \begin{table*}[hbtp]
%     \caption{Survey of reported beamforming work in sub-mmWave band}
%     \setlength{\tabcolsep}{5pt}
%     \centering
% \resizebox{0.7\textwidth}{!}{
%      \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||} 
%      \hline 
%     Paper & Frequency & Environment & Type & Bandwidth & Parameters & Target Applications & General Aspect\\
%      \hline 
%      \hline
%     \end{tabular}}
%     \label{tab:survey_sub6}
% \end{table*}

%LIMITATIONS OF 6GHZ COMMUNICATIONS AND NEED FOR MMWAVE COMM.

%Such a large data transfer volume at short contact times can quickly saturate the sub-6 GHz band.

% % \subsubsection{Sub-30 GHz}
% 5G speeds will range from ~50 Mbit/s to over a gigabit/s.[20] The fastest 5G is known as mmWave. As of July 3, 2019, mmWave had a top speed of 1.8 Gbit/s[21] on AT\&T's 5G network.

\subsection{Using the mmWave Band}
The two standardized mmWave bands in 5G NR are n259 (39.5-43.5 GHz) and n260 (37-40 GHz). Utilization of these two bands provides even higher spectral efficiency than all sub-30 GHz bands. using mMIMO and higher order modulation techniques, the mmWave can offer higher data rates in 5G compliant wireless communication systems, than the sub-30 GHz ones~\cite{Ghafoor_2020}. 

With the glimpse on the bands, we next present a comparison analysis of the state-of-the-art of last 5 years for beamforming techniques in those bands in Tab.~\ref{tab:survey_mmwave}. The focus of the survey is not to review the existing beamforming techniques, rather mainly to find the trend in beamforming for 5G/6G  standards and shortcoming in those. Hence in the comparison analysis we present different types of challenges and difficulties for conventional beamforming in sub-mmWave and mmWave bands for 5G NR standard. From the analysis, it is clear most of the state-of-the-art is focused on improving the analog beamforming in the higher frequencies of 5G and validating with simulation results. However, the problem of dealing with the overhead of analog beamforming is still lingering challenge to overcome with the conventional methods~\cite{Ghafoor_2020}. 

%DISCUSS WHY WE NEED TO AID THE BEAMFORMING FOR MMWAVE. 
However, to support the multipath propagation, the beamforming aspect in mmWave band is also categorized as open-loop (implicit) and close-loop (explicit) beamforming~\cite{Lou_2013, Clerckx_2010} for a real-world deployment. In open-loop beamforming the transmitter performs a on-the-fly channel sounding process to calculate the antenna weight vectors which gives lower overhead. However, the bottleneck is to find the perfect channel sounding process considered the multipath situation. Whereas, the closed loop strategy works by the receiver estimating the channel and sending a feedback to the receiver~\cite{Kutty_2016}. This feedback communication generally happen in a separate band than the original mmWave communication. Overall, the close-loop beamforming outperforms the open-loop method, albeit the higher computational complexity and overhead.

\begin{table*}[hbtp]
    \setlength{\tabcolsep}{5pt}
    \centering
\resizebox{1.0\textwidth}{!}{
     \begin{tabular}{c|c|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{3cm}|p{2cm}|p{2cm}|p{2cm}} 
          \specialrule{.2em}{.1em}{.1em}  
          \rowcolor{lightgray}
    {\bf Paper} & {\bf Year} & {\bf Frequency} & {\bf Compatible Standards} &{\bf Beamforming Type} & {\bf Target} & {\bf Assumptions} & {\bf Quantified Parameters} & {\bf Shortcomings}\\     \specialrule{.2em}{.1em}{.1em} 
    Wu {\em et al.}~\cite{Wu_2017}  & 2017 & 28GHz & 5G NR & Hybrid & Non-orthogonal multiple access (NOMA) based hybrid beamforming design & Analog beamforming at UEs & Sum capacity & Simulation results in constrained settings\\\hline
    Jo {\em et al.}~\cite{Jo_2017} & 2017 & 60 GHz & 5G NR and IEEE 802.ad/ay & Hybrid & Dual polarization for mmWave beamforming systems & Hybrid beamforming restricted to dual polarization& Received power and MIMO channel capacity, channel frequncy response & Stationary testbed\\\hline
    Sun {\em et al.}~\cite{Sun_2018} & 2018 & 28 GHz & 5G NR& Hybrid & Beamforming schemes for multi-cell multi-user multi-stream mmWave communication& All UEs use all available RF chains &Spectral efficiency, average power&Simulation with basic channel modeling\\\hline
    Yang {\em et al.}~\cite{Yang_2018} & 2018 &28 GHz&5G NR&Digital&Design  64-channel mMIMO transceiver with a fully digital beamforming architecture& 2-D antenna array with 16 columns (horizontal direction) and 4 rows (vertical direction)&Phase noise, gain, power, throughout &cost of digital baseband processing part\\\hline
    Xiao {\em et al.}~\cite{Xiao_2018} & 2018 &mmWave&5G NR&Analog&Assign beamforming vector weight to accommodate two users simultaneously subject to an analog beamforming structure using  non-orthogonal multiple access& Suboptimal solution&Sum rate, power allocation, beam gain&Simulation results\\\hline
      Bai {\em et al.}~\cite{Bai_2018} & 2018 &mmWave&5G NR&Analog&Cooperative multiuser beamforming method for energy-efficient transmissions in mmWave distributed antenna systems&BS has the full CSI &Transmit power&Constrained simulation results\\\hline
     Zhu {\em et al.}~\cite{Zhu_2018} & 2018 &mmWave&5G NR&Analog&Joint power control and beamforming problem for mmWave-NOMA system&Sub-optimal solution&Beam gain, bit rate&Constrained simulation\\\hline
      Zhu {\em et al.}~\cite{Zhu_2019} & 2019 &mmWave&5G NR&Analog& Joint Tx-Rx beamforming and power allocation to maximize the achievable sum rate for mmWave-NOMA  &Sub-optimal solution&Sum rate, power allocation, channel gain&Constrained simulation\\\hline
    Zhou {\em et al.}~\cite{Zhou_2019} & 2019 &6 GHz &5G NR&Analog&Beamforming to reduce the UE localization error for millimeter-wave MIMO systems&Assumption on convergence analysis& Localization RMSE, beamforming refinement gain&Simulation on static UEs\\\hline
      Mismar {\em et al.}~\cite{Mismar_2020} & 2020 &Sub-6 GHz and mmWave&5G NR&Analog& Joint optimization of beamforming, power control, and interference coordination to maximize the SINR&BS selects transmit power and beamforming vectors from finite set&Sum rate, transmit power&Constrained simulation results\\\specialrule{.2em}{.1em}{.1em} 

    \end{tabular}}
       \caption{Survey of reported beamforming work in last 5 years for 5G/6G.}
               \label{tab:survey_mmwave}
\end{table*}

% Non-orthogonal multiple access based hybrid beamforming in 5G mmWave systems - \cite{Wu_2017}
% Exploitation of Dual-Polarization Diversity for 5G Millimeter-Wave MIMO Beamforming Systems - \cite{Jo_2017}
% Hybrid beamforming for 5G millimeter-wave multi-cell networks - \cite{Sun_2018}
% Digital Beamforming-Based mMIMO Transceiver for 5G Millimeter-Wave Communications - \cite{Yang_2018}
% Joint Power Allocation and Beamforming for Non-Orthogonal Multiple Access (NOMA) in 5G Millimeter Wave Communications - \cite{Xiao_2018}
% Cooperative Multiuser Beamforming in mmWave Distributed Antenna Systems - \cite{Bai_2018}
% Joint Power Control and Beamforming for Uplink Non-Orthogonal Multiple Access in 5G Millimeter-Wave Communications - \cite{Zhu_2018}
% Joint Tx-Rx Beamforming and Power Allocation for 5G Millimeter-Wave Non-Orthogonal Multiple Access Networks - \cite{Zhu_2019}
%Successive Localization and Beamforming in 5G mmWave MIMO Communication Systems - \cite{Zhou_2019} 
% Deep Reinforcement Learning for 5G Networks: Joint Beamforming, Power Control, and Interference Coordination - \cite{Mismar_2020}






